Towards Zero-Shot Personalized Table-to-Text Generation with Contrastive Persona Distillation

Existing neural methods have shown great potentials towards generating informative text from structured tabular data as well as maintaining high content fidelity. However, few of them shed light on generating personalized expressions, which often requires well-aligned persona-table-text datasets that are difficult to obtain. To overcome these obstacles, we explore personalized table-to-text generation under a zero-shot setting, by assuming no well-aligned persona-table-text triples are required during training. To this end, we firstly collect a set of unpaired persona information and then propose a semi-supervised approach with contrastive persona distillation (S2P-CPD) to generate personalized context. Specifically, tabular data and persona information are firstly represented as latent variables separately. Then, we devise a latent space fusion technique to distill persona information into the table representation. Besides, a contrastive-based discriminator is employed to guarantee the style consistency between the generated context and its corresponding persona. Experimental results on two benchmarks demonstrate S2P-CPD's ability on keeping both content fidelity and personalized expressions.

==> relatedwork.tex <==
\section{Related Work}

Our work is related to two research branches: Data-to-text Generation, and Personalized Content Generation.

\textbf{\textit{Data-to-text Generation}}
Data-to-text generation has been widely studied~\cite{moryossef-etal-2019-step,puduppully2019data,zhao-etal-2020-bridging,wiseman-etal-2021-data}, which involves generating natural language from structured data. Most of the previous work has formulated data-to-text generation into two sub-tasks: content selection~\cite{puduppully2019AAAI} and surface realization~\cite{moryossef-etal-2019-step}. Many efforts have been made to improve the fidelity of generated text to the record content, through sophisticated neural architectures. Prior to deep learning era, traditional systems are primarily built on template-based rules~\cite{van-der-lee-etal-2018-automated}, which carefully learns the alignment between data and content. Recently, with the development of deep learning, attention has been gradually shifted to end-to-end neural generation models, which achieve significant performances. Another line of work attempts to use external knowledge to improve the quality of generated text. These methods allow generation from an expanded external knowledge base that may contain information not relevant to the input table~\cite{chen2019towards,chen2020kgpt}. Comparatively, our setting requires the generated text to be faithful to the input table.
Regarding datasets, most previous methods are trained and evaluated on large-scaled datasets like WebNLG~\cite{gardent2017webnlg}, WikiBio~\cite{lebret2016wiki}, and TOTTO~\cite{parikh2020totto}. However, both of these datasets mainly focus on the content fidelity and do not consider the personalized content. Considering the application of data-to-text generation task in many fields, personalized expressions are also very important. So, to the best of our knowledge, we are the first to crowd-source and provide user profile tailored data-to-text dataset. 


% In terms of stylized generation, one related parallel work is \cite{lin2020data}. However, our method is completely different from theirs. Specifically,
% \cite{lin2020data} develop a confidence oriented
% decoder that assigns a confidence score to each
% target position to reduce the unfaithful information. 


\textbf{\textit{Personalized Content Generation}} Personalized content generation has attracted research interest in various domains, e.g., E-commerce~\cite{zhao2019dynamic,chen2019fine}, the automatic generation of marketing messages \cite{roy2015automated}, persuasive message \cite{ding2016personalized}, poetry generation~\cite{shen2020compose}, and argument generation \cite{carenini2006generating}. With the support of user preferences, the effectiveness has increases. Recently, \cite{krishna2018vocabulary} presented a framework for the summary generation that takes into consideration the linguistic preferences of the specific audience.
% As for computer-based research,
\cite{reichelt2014talk} showed that personalized information of learning materials can increase motivation and learning outcomes. \cite{zander2015does} studied the effect of personalization on students' attention allocation using some eye-tracking methods, and find that the personalized parts of reading materials are more attractive. In the field of E-commerce, %\cite{chen2019towards} proposed to incorporate the customer profile and external product knowledge from Wikipedia to generate the product description.
\cite{elad2019learning} proposed an extractive method to select sentences and then generate personalized product description. \cite{chen2019pog} built a bridge between personalized outfit generation and recommendation by considering both user preferences and individual items. 
To the best of our knowledge, our method takes the first attempt to introduce personalized aspects for data-to-text generation task.


